Attesting Distributional Properties of Training Data for Machine Learning

The success of machine learning (ML) has been accompanied by increased concerns about its trustworthiness. Several jurisdictions are preparing ML regulatory frameworks. One such concern is ensuring that model training data has desirable distributional properties for certain sensitive attributes. For example, draft regulations indicate that model trainers are required to show that training datasets have specific distributional properties, such as reflecting diversity of the population. We propose the notion of property attestation allowing a prover (e.g., model trainer) to demonstrate relevant distributional properties of training data to a verifier (e.g., a customer) without revealing the data. We present an effective hybrid property attestation combining property inference with cryptographic mechanisms.

==> tables/misc/tab_arxiv_whitebox_attestation.tex <==
% \begin{table*}
% \caption{TAR and TRR for \arxiv dataset with 1\%, 5\% and 10\% thresholds for FAR and FRR across different $p_{claim}$.}
% \begin{center}
% \begin{tabular}{ c|c|c|c|c|c|c } 
%  \toprule
%  &  \multicolumn{3}{c|}{\textbf{FAR-TAR Curve}} & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
%  \textbf{$p_{claim}$}  & \textbf{TAR @ 1\% FAR}  & \textbf{TAR @ 5\% FAR} & \textbf{TAR @ 10\% FAR} & \textbf{TRR @ 1\% FRR}  & \textbf{TRR @ 5\% FRR} & \textbf{TRR @ 10\% FRR}\\ 
%  \toprule
% 9  & 0.95 & 0.99 & 1.00  & 0.96 & 0.99 & 0.99 \\ 
% 10  & 0.93 & 0.98 & 1.00  & 0.94 & 0.98 & 0.99 \\ 
% 11  & 0.14 & 0.40 & 0.57  & 0.82 & 0.83 & 0.84\\ 
% 12  & 0.45 & 0.72 & 0.87 & 0.74 & 0.82 & 0.88\\ 
% 13  & 0.31 & 0.59 & 0.78  & 0.71 & 0.80 & 0.84\\ 
% 14  & 0.88 & 0.95 & 0.98  & 0.87 & 0.95 & 0.98\\ 
% 15 & 0.88 & 0.96 & 0.99 & 0.92 & 0.96 & 0.98\\ 
% 16  & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00\\ 
% 17 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00\\ 
%  \bottomrule
% \end{tabular}
% \end{center}
% \label{tab:arxiv}
% \end{table*}


\begin{table}
\caption{TAR and TRR for \arxiv dataset with 5\% thresholds for FAR, FRRacross different $p_{claim}$ windows. The $p_{claim}$ value within the window is indicated in \textbf{bold}.}
\begin{center}
\begin{tabular}{ c|c|c|c} 
 \toprule
 \textbf{$p_{claim}$ Range}  & \textbf{TAR @ 5\% FAR}  &  \textbf{TRR @ 5\% FRR} & \textbf{EER}\\ 
 \toprule
\{\textbf{9}, 10\}  & 0.99 & 0.99 & 0.02 \\ 
\{9, \textbf{10}, 11\} & 0.98 & 0.98 & 0.03 \\ 
\{10, \textbf{11}, 12\} & 0.40 & 0.83 & 0.15\\ 
\{11, \textbf{12}, 13\} & 0.72 & 0.82 & 0.13\\ 
\{12, \textbf{13}, 14\} & 0.59 & 0.80 & 0.13 \\ 
\{13, \textbf{14}, 15\} & 0.95 & 0.95 & 0.05\\ 
\{14, \textbf{15}, 16\} & 0.96 & 0.96 & 0.05\\ 
\{15, \textbf{16}, 17\} & 1.00 & 1.00 & 0.00 \\ %4e-3
\{16, \textbf{17}\} & 1.00 & 1.00 & 0.00\\ %6e-4
 \bottomrule
\end{tabular}
\end{center}
\label{tab:arxiv}
\end{table}

==> tables/misc/tab_boneage_whitebox_attestation.tex <==
% \begin{table*}
% \caption{TAR and TRR for \boneage dataset with 1\%, 5\% and 10\% thresholds for FAR and FRR across different $p_{claim}$.}
% \begin{center}
% \begin{tabular}{ c|c|c|c|c|c|c } 
%  \toprule
%  &  \multicolumn{3}{c|}{\textbf{FAR-TAR Curve}} & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
%  \textbf{$p_{claim}$} & \textbf{TAR @ 1\% FAR}  & \textbf{TAR @ 5\% FAR} & \textbf{TAR @ 10\% FAR}  & \textbf{TRR @ 1\% FRR}  & \textbf{TRR @ 5\% FRR} & \textbf{TRR @ 10\% FRR}\\ 
%  \toprule
% 0.20 & 0.80 & 0.93 & 0.97  & 0.86 & 0.93 & 0.97 \\ 
% 0.30 & 0.86 & 0.96 & 0.98 & 0.89 & 0.95 & 0.97 \\ 
% 0.40 & 0.64 & 0.76 & 0.81  & 0.47 & 0.56 & 0.65\\ 
% 0.50 & 0.38 & 0.50 & 0.56  & 0.43 & 0.53 & 0.61\\ 
% 0.60 & 0.29 & 0.35 & 0.41  & 0.67 & 0.73 & 0.76\\ 
% 0.70 & 0.89 & 0.95 & 0.98  & 0.89 & 0.95 & 0.98\\ 
% 0.80 & 0.34 & 0.65 & 0.91  & 0.80 & 0.87 & 0.90\\ 
%  \bottomrule
% \end{tabular}
% \end{center}
% \label{tab:boneage}
% \end{table*}

\begin{table}
\caption{TAR and TRR for \boneage dataset with 5\% thresholds for FAR and FRR across different $p_{claim}$ windows. The $p_{claim}$ value within the window is indicated in \textbf{bold}.}
\begin{center}
\begin{tabular}{ c|c|c|c } 
 \toprule
 \textbf{$p_{claim}$ Range} & \textbf{TAR @ 5\% FAR}  & \textbf{TRR @ 5\% FRR} & \textbf{EER}\\ 
 \toprule
\{\textbf{0.20}, 0.30\} & 0.93 & 0.93 & 0.06 \\ 
\{0.20, \textbf{0.30}, 0.40\} & 0.96 & 0.95 & 0.05\\ 
\{0.30, \textbf{0.40}, 0.50\} & 0.76 & 0.56 & 0.16\\ 
\{0.40, \textbf{0.50}, 0.60\} & 0.50 & 0.53 & 0.24\\ 
\{0.50, \textbf{0.60}, 0.70\} & 0.35 & 0.73 & 0.22\\ 
\{0.60, \textbf{0.70}, 0.80\} & 0.95 & 0.95 & 0.05\\ 
\{0.70, \textbf{0.80}\} & 0.65 & 0.87 & 0.10\\ 
 \bottomrule
\end{tabular}
\end{center}
\label{tab:boneage}
\end{table}

==> tables/misc/tab_censusRace_whitebox_attestation.tex <==
% \begin{table*}
% \caption{TAR and TRR for \racecensus dataset with 1\%, 5\% and 10\% thresholds for FAR and FRR across different $p_{claim}$.}
% \begin{center}
% \begin{tabular}{ c|c|c|c|c|c|c} 
%  \toprule
%  &  \multicolumn{3}{c|}{\textbf{FAR-TAR Curve}}
%  & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
%  {\textbf{$p_{claim}$}} & 
% {\textbf{TAR @ 1\% FAR}}  & 
%  {\textbf{TAR @ 5\% FAR}} & 
%  {\textbf{TAR @ 10\% FAR}} & 
%  {\textbf{TRR @ 1\% FRR}}  & 
%  {\textbf{TRR @ 5\% FRR}} & 
%  {\textbf{TRR @ 10\% FRR}} &
%  {\textbf{EER}}\\ 
%  \toprule
% 0.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.0\\ 
% 0.10 & 0.08 & 0.34 & 0.57 & 0.53 & 0.63 & 0.69 & 0.20 \\
% 0.20 & 0.47 & 0.72 & 0.84 & 0.70 & 0.81 & 0.86 & 0.13\\ 
% 0.30 & 0.01 & 0.04 & 0.12 & 0.27 & 0.42 & 0.51 & 0.33\\ 
% 0.40 & 0.07 & 0.19 & 0.32 & 0.17 & 0.32 & 0.43 & 0.32\\ 
% 0.50 & 0.04 & 0.15 & 0.23 & 0.04 & 0.14 & 0.22 & 0.40\\ 
% 0.60 & 0.02 &  0.07 & 0.13 & 0.05 & 0.13 & 0.22 & 0.42\\
% 0.70 & 0.06 & 0.24 & 0.44 & 0.34 & 0.52 & 0.63 & 0.23\\ 
% 0.80 & 0.55 & 0.80 & 0.89 & 0.67 & 0.83 & 0.89 & 0.11\\ 
% 0.90 & 0.34 & 0.64 & 0.79 & 0.44 & 0.72 & 0.81 & 0.15\\ 
% 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.00\\ 
%  \bottomrule
% \end{tabular}
% \end{center}
% \label{tab:censusrace}
% \end{table*}

\begin{table}
\caption{TAR and TRR for \racecensus dataset with 5\% thresholds for FAR, FRR, EER across different $p_{claim}$ windows. The $p_{claim}$ value within the window is indicated in \textbf{bold}.}
\begin{center}
\begin{tabular}{ c|c|c|c} 
 \toprule
 % &  \multicolumn{}{c|}{\textbf{FAR-TAR Curve}}
 % & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
 {\textbf{$p_{claim}$}} & 
 {\textbf{TAR @ 5\% FAR}} & 
 {\textbf{TRR @ 5\% FRR}} & 
 {\textbf{EER}}\\ 
 \toprule
 \{\textbf{0.00}\} & 1.00 & 1.00 & 0.00\\ 
 \{0.00, \textbf{0.10}, 0.20\} & 0.34 & 0.63 & 0.20 \\
 \{0.10, \textbf{0.20}, 0.30\} & 0.72 & 0.81 & 0.13\\ 
 \{0.20, \textbf{0.30}, 0.40\} & 0.04 & 0.42 & 0.33\\ 
 \{0.30, \textbf{0.40}, 0.50\} & 0.19 & 0.32 & 0.32\\ 
 \{0.40, \textbf{0.50}, 0.60\} & 0.15 & 0.14 & 0.40\\ 
 \{0.50, \textbf{0.60}, 0.70\} & 0.07 & 0.13 & 0.42\\
 \{0.60, \textbf{0.70}, 0.80\} & 0.24 & 0.52 & 0.23\\ 
 \{0.70, \textbf{0.80}, 0.90\} & 0.80 & 0.83 & 0.11\\ 
 \{0.80, \textbf{0.90}, 1.00\} & 0.64 & 0.72 & 0.15\\ 
 \{\textbf{1.00}\} & 1.00 & 1.00 & 0.00\\ 
 \bottomrule
\end{tabular}
\end{center}
\label{tab:censusrace}
\end{table}


==> tables/misc/tab_censusSex_whitebox_attestation.tex <==
% \begin{table*}
% \caption{TAR and TRR for \sexcensus dataset with 1\%, 5\% and 10\% thresholds for FAR and FRR across different $p_{claim}$.}
% \begin{center}
% \begin{tabular}{ c|c|c|c|c|c|c} 
%  \toprule
%  &  \multicolumn{3}{c|}{\textbf{FAR-TAR Curve}}
%  & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
%  {\textbf{$p_{claim}$}} & 
% {\textbf{TAR @ 1\% FAR}}  & 
%  {\textbf{TAR @ 5\% FAR}} & 
%  {\textbf{TAR @ 10\% FAR}} & 
%  {\textbf{TRR @ 1\% FRR}}  & 
%  {\textbf{TRR @ 5\% FRR}} & 
%  {\textbf{TRR @ 10\% FRR}} & 
%  {\textbf{EER}}\\ 
%  \toprule
% 0.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.00\\ 
% 0.10 & 0.20 & 0.41 & 0.52 & 0.21 & 0.40 & 0.52 & 0.25\\ 
% 0.20 & 0.44 & 0.64 & 0.74 & 0.42 & 0.64 & 0.77 & 0.16\\ 
% 0.30 & 0.08 & 0.24 & 0.39 & 0.21 & 0.37 & 0.48 & 0.29\\ 
% 0.40 & 0.03 & 0.10 & 0.22 & 0.11 & 0.21 & 0.31 & 0.38\\ 
% 0.50 & 0.07 & 0.15 & 0.26 & 0.05 & 0.14 & 0.24 & 0.39\\ 
% 0.60 & 0.03 &  0.12 & 0.20 & 0.03 & 0.12 & 0.20 & 0.41\\
% 0.70 & 0.02 & 0.10 & 0.21 & 0.10 & 0.23 & 0.32 & 0.36\\ 
% 0.80 & 0.32 & 0.53 & 0.66 & 0.37 & 0.58 & 0.69 & 0.20\\ 
% 0.90 & 0.27 & 0.50 & 0.66 & 0.38 & 0.59 & 0.69 & 0.19\\ 
% 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.00\\ 
%  \bottomrule
% \end{tabular}
% \end{center}
% \label{tab:censussex}
% \end{table*}


\begin{table}
\caption{TAR and TRR for \sexcensus dataset with 5\% thresholds for FAR, FRR, EER across different $p_{claim}$ windows. The $p_{claim}$ value within the window is indicated in \textbf{bold}.}
\begin{center}
\begin{tabular}{ c|c|c|c} 
 \toprule
 % &  \multicolumn{3}{c|}{\textbf{FAR-TAR Curve}}
 % & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
 {\textbf{$p_{claim}$}} & 
% {\textbf{TAR @ 1\% FAR}}  & 
 {\textbf{TAR @ 5\% FAR}} & 
 % {\textbf{TAR @ 10\% FAR}} & 
 % {\textbf{TRR @ 1\% FRR}}  & 
 {\textbf{TRR @ 5\% FRR}} & 
 % {\textbf{TRR @ 10\% FRR}} & 
 {\textbf{EER}}\\ 
 \toprule
 \{\textbf{0.00}\} & 1.00 & 1.00 & 0.00\\ 
\{0.00, \textbf{0.10}, 0.20\} & 0.41 & 0.40 & 0.25\\ 
 \{0.10, \textbf{0.20}, 0.30\} & 0.64 & 0.64 & 0.16\\ 
\{0.20, \textbf{0.30}, 0.40\} & 0.24 & 0.37 & 0.29\\ 
\{0.30, \textbf{0.40}, 0.50\} & 0.10 & 0.21 & 0.38\\ 
\{0.40, \textbf{0.50}, 0.60\} & 0.15 & 0.14 & 0.39\\ 
\{0.50, \textbf{0.60}, 0.70\} & 0.12 & 0.12 & 0.41\\
\{0.60, \textbf{0.70}, 0.80\} & 0.10 & 0.23 & 0.36\\ 
\{0.70, \textbf{0.80}, 0.90\} & 0.53 & 0.58 & 0.20\\ 
\{0.80, \textbf{0.90}, 1.00\} & 0.50 & 0.59 & 0.19\\ 
 \{\textbf{1.00}\} & 1.00 & 1.00 & 0.00\\ 
 \bottomrule
\end{tabular}
\end{center}
\label{tab:censussex}
\end{table}

==> tables/tab_effectiveness_test_new.tex <==
\begin{table*}[!htb]
\setlength\tabcolsep{1pt}
\footnotesize
\caption{TAR and TRR for \racecensus dataset with 5\% thresholds for FAR, FRR along with EER across different \preq windows on \verifiertestdata. The \preq value within the window is indicated in \textbf{bold}. Edge \preq values have higher effectiveness than middle \preq values due to difference in distinguishable in first layer parameters~\cite{suripropinf}.}
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \caption{\arxiv}
\begin{tabular}{ c|c|c|c} 
 \toprule
 \textbf{\preq Range}  & \textbf{TAR @ 5\% FAR}  &  \textbf{TRR @ 5\% FRR} & \textbf{EER}\\ 
 \toprule
\{\textbf{9}, 10\}  & 0.99 & 0.98 & 0.03 \\ 
\{9, \textbf{10}, 11\} & 0.98 & 0.98 & 0.04 \\ 
\{10, \textbf{11}, 12\} & 0.39 & 0.83 & 0.15\\ 
\{11, \textbf{12}, 13\} & 0.71 & 0.83 & 0.12\\ 
\{12, \textbf{13}, 14\} & 0.61 & 0.82 & 0.13 \\ 
\{13, \textbf{14}, 15\} & 0.97 & 0.97 & 0.04\\ 
\{14, \textbf{15}, 16\} & 0.96 & 0.95 & 0.05\\ 
\{15, \textbf{16}, 17\} & 1.00 & 1.00 & 0.00 \\ %4e-3
\{16, \textbf{17}\} & 1.00 & 1.00 & 0.00\\ %6e-4
 \bottomrule
\end{tabular}
    \end{subtable}%  
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \caption{\boneage}
\begin{tabular}{ c|c|c|c } 
 \toprule
 \textbf{\preq Range} & \textbf{TAR @ 5\% FAR}  & \textbf{TRR @ 5\% FRR} & \textbf{EER}\\ 
 \toprule
\{\textbf{0.20}, 0.30\} & 0.93 & 0.93 & 0.06 \\ 
\{0.20, \textbf{0.30}, 0.40\} & 0.96 & 0.95 & 0.05\\ 
\{0.30, \textbf{0.40}, 0.50\} & 0.76 & 0.56 & 0.16\\ 
\{0.40, \textbf{0.50}, 0.60\} & 0.50 & 0.53 & 0.24\\ 
\{0.50, \textbf{0.60}, 0.70\} & 0.35 & 0.73 & 0.22\\ 
\{0.60, \textbf{0.70}, 0.80\} & 0.95 & 0.95 & 0.05\\ 
\{0.70, \textbf{0.80}\} & 0.65 & 0.87 & 0.10\\ 
 \bottomrule
\end{tabular}
    \end{subtable}\\
\begin{subtable}[t]{.5\linewidth}
\centering
 \caption{\sexcensus}
\begin{tabular}{ c|c|c|c} 
 \toprule
 {\textbf{\preq Range}} & 
 {\textbf{TAR @ 5\% FAR}} & 
 {\textbf{TRR @ 5\% FRR}} & 
 {\textbf{EER}}\\ 
 \toprule
 \{\textbf{0.00}\} & 1.00 & 1.00 & 0.00\\ 
\{0.00, \textbf{0.10}, 0.20\} & 0.41 & 0.40 & 0.25\\ 
 \{0.10, \textbf{0.20}, 0.30\} & 0.65 & 0.66 & 0.16\\ 
\{0.20, \textbf{0.30}, 0.40\} & 0.23 & 0.37 & 0.29\\ 
\{0.30, \textbf{0.40}, 0.50\} & 0.10 & 0.23 & 0.38\\ 
\{0.40, \textbf{0.50}, 0.60\} & 0.16 & 0.13 & 0.39\\ 
\{0.50, \textbf{0.60}, 0.70\} & 0.11 & 0.13 & 0.41\\
\{0.60, \textbf{0.70}, 0.80\} & 0.10 & 0.21 & 0.37\\ 
\{0.70, \textbf{0.80}, 0.90\} & 0.53 & 0.56 & 0.20\\ 
\{0.80, \textbf{0.90}, 1.00\} & 0.52 & 0.57 & 0.20\\ 
 \{\textbf{1.00}\} & 1.00 & 1.00 & 0.00\\ 
 \bottomrule
\end{tabular}
    \end{subtable}%
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \caption{\racecensus}
\begin{tabular}{ c|c|c|c} 
 \toprule
 % &  \multicolumn{}{c|}{\textbf{FAR-TAR Curve}}
 % & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
 {\textbf{\preq Range}} & 
 {\textbf{TAR @ 5\% FAR}} & 
 {\textbf{TRR @ 5\% FRR}} & 
 {\textbf{EER}}\\ 
 \toprule
 \{\textbf{0.00}\} & 1.00 & 1.00 & 0.00\\ 
 \{0.00, \textbf{0.10}, 0.20\} & 0.35 & 0.67 & 0.20 \\
 \{0.10, \textbf{0.20}, 0.30\} & 0.68 & 0.80 & 0.13\\ 
 \{0.20, \textbf{0.30}, 0.40\} & 0.04 & 0.41 & 0.33\\ 
 \{0.30, \textbf{0.40}, 0.50\} & 0.19 & 0.31 & 0.31\\ 
 \{0.40, \textbf{0.50}, 0.60\} & 0.15 & 0.15 & 0.40\\ 
 \{0.50, \textbf{0.60}, 0.70\} & 0.08 & 0.13 & 0.42\\
 \{0.60, \textbf{0.70}, 0.80\} & 0.25 & 0.53 & 0.23\\ 
 \{0.70, \textbf{0.80}, 0.90\} & 0.79 & 0.83 & 0.11\\ 
 \{0.80, \textbf{0.90}, 1.00\} & 0.65 & 0.72 & 0.15\\ 
 \{\textbf{1.00}\} & 1.00 & 1.00 & 0.00\\ 
 \bottomrule
\end{tabular}
    \end{subtable}
\label{tab:effectiveness}
\end{table*}

==> tables/tab_effectiveness_test_previous.tex <==
\begin{table*}[b]
\setlength\tabcolsep{1pt}
\footnotesize
\caption{TAR and TRR for \racecensus dataset with 5\% thresholds for FAR, FRR along with EER across different \preq windows. The \preq value within the window is indicated in \textbf{bold}. Edge \preq values have higher effectiveness than middle \preq values due to difference in distinguishable in first layer parameters~\cite{suripropinf}.}
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \caption{\arxiv}
\begin{tabular}{ c|c|c|c} 
 \toprule
 \textbf{\preq Range}  & \textbf{TAR @ 5\% FAR}  &  \textbf{TRR @ 5\% FRR} & \textbf{EER}\\ 
 \toprule
\{\textbf{9}, 10\}  & 0.99 & 0.99 & 0.02 \\ 
\{9, \textbf{10}, 11\} & 0.98 & 0.98 & 0.03 \\ 
\{10, \textbf{11}, 12\} & 0.40 & 0.83 & 0.15\\ 
\{11, \textbf{12}, 13\} & 0.72 & 0.82 & 0.13\\ 
\{12, \textbf{13}, 14\} & 0.59 & 0.80 & 0.13 \\ 
\{13, \textbf{14}, 15\} & 0.95 & 0.95 & 0.05\\ 
\{14, \textbf{15}, 16\} & 0.96 & 0.96 & 0.05\\ 
\{15, \textbf{16}, 17\} & 1.00 & 1.00 & 0.00 \\ %4e-3
\{16, \textbf{17}\} & 1.00 & 1.00 & 0.00\\ %6e-4
 \bottomrule
\end{tabular}
    \end{subtable}%  
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \caption{\boneage}
\begin{tabular}{ c|c|c|c } 
 \toprule
 \textbf{\preq Range} & \textbf{TAR @ 5\% FAR}  & \textbf{TRR @ 5\% FRR} & \textbf{EER}\\ 
 \toprule
\{\textbf{0.20}, 0.30\} & 0.93 & 0.93 & 0.06 \\ 
\{0.20, \textbf{0.30}, 0.40\} & 0.96 & 0.95 & 0.05\\ 
\{0.30, \textbf{0.40}, 0.50\} & 0.76 & 0.56 & 0.16\\ 
\{0.40, \textbf{0.50}, 0.60\} & 0.50 & 0.53 & 0.24\\ 
\{0.50, \textbf{0.60}, 0.70\} & 0.35 & 0.73 & 0.22\\ 
\{0.60, \textbf{0.70}, 0.80\} & 0.95 & 0.95 & 0.05\\ 
\{0.70, \textbf{0.80}\} & 0.65 & 0.87 & 0.10\\ 
 \bottomrule
\end{tabular}
    \end{subtable}\\
\begin{subtable}[t]{.5\linewidth}
\centering
 \caption{\sexcensus}
\begin{tabular}{ c|c|c|c} 
 \toprule
 {\textbf{\preq Range}} & 
 {\textbf{TAR @ 5\% FAR}} & 
 {\textbf{TRR @ 5\% FRR}} & 
 {\textbf{EER}}\\ 
 \toprule
 \{\textbf{0.00}\} & 1.00 & 1.00 & 0.00\\ 
\{0.00, \textbf{0.10}, 0.20\} & 0.41 & 0.40 & 0.25\\ 
 \{0.10, \textbf{0.20}, 0.30\} & 0.64 & 0.64 & 0.16\\ 
\{0.20, \textbf{0.30}, 0.40\} & 0.24 & 0.37 & 0.29\\ 
\{0.30, \textbf{0.40}, 0.50\} & 0.10 & 0.21 & 0.38\\ 
\{0.40, \textbf{0.50}, 0.60\} & 0.15 & 0.14 & 0.39\\ 
\{0.50, \textbf{0.60}, 0.70\} & 0.12 & 0.12 & 0.41\\
\{0.60, \textbf{0.70}, 0.80\} & 0.10 & 0.23 & 0.36\\ 
\{0.70, \textbf{0.80}, 0.90\} & 0.53 & 0.58 & 0.20\\ 
\{0.80, \textbf{0.90}, 1.00\} & 0.50 & 0.59 & 0.19\\ 
 \{\textbf{1.00}\} & 1.00 & 1.00 & 0.00\\ 
 \bottomrule
\end{tabular}
    \end{subtable}%
    \begin{subtable}[t]{.5\linewidth}
      \centering
        \caption{\racecensus}
\begin{tabular}{ c|c|c|c} 
 \toprule
 % &  \multicolumn{}{c|}{\textbf{FAR-TAR Curve}}
 % & \multicolumn{3}{c}{\textbf{FRR-TRR Curve}} \\
 {\textbf{\preq Range}} & 
 {\textbf{TAR @ 5\% FAR}} & 
 {\textbf{TRR @ 5\% FRR}} & 
 {\textbf{EER}}\\ 
 \toprule
 \{\textbf{0.00}\} & 1.00 & 1.00 & 0.00\\ 
 \{0.00, \textbf{0.10}, 0.20\} & 0.34 & 0.63 & 0.20 \\
 \{0.10, \textbf{0.20}, 0.30\} & 0.72 & 0.81 & 0.13\\ 
 \{0.20, \textbf{0.30}, 0.40\} & 0.04 & 0.42 & 0.33\\ 
 \{0.30, \textbf{0.40}, 0.50\} & 0.19 & 0.32 & 0.32\\ 
 \{0.40, \textbf{0.50}, 0.60\} & 0.15 & 0.14 & 0.40\\ 
 \{0.50, \textbf{0.60}, 0.70\} & 0.07 & 0.13 & 0.42\\
 \{0.60, \textbf{0.70}, 0.80\} & 0.24 & 0.52 & 0.23\\ 
 \{0.70, \textbf{0.80}, 0.90\} & 0.80 & 0.83 & 0.11\\ 
 \{0.80, \textbf{0.90}, 1.00\} & 0.64 & 0.72 & 0.15\\ 
 \{\textbf{1.00}\} & 1.00 & 1.00 & 0.00\\ 
 \bottomrule
\end{tabular}
    \end{subtable}
\label{tab:effectiveness}
\end{table*}

==> tables/tab_efficiency.tex <==
\begin{table}[!htb]
\setlength\tabcolsep{1pt}
\scriptsize
\caption{\verifier's one-time cost for inference-based attestation: Total training time(s) on a single GPU for 10 attestation classifiers and 1000 shadow models.}
\begin{center}
\begin{tabular}{ c|c|c } 
 \toprule
 \textbf{Dataset} &
 \textbf{\attclf} & \textbf{Shadow Models}\\
 \toprule
 \textbf{\boneage} & 12000 & 10400\\
 \midrule
\textbf{\arxiv} & 725 & 7400\\
 \midrule
\textbf{\sexcensus} & \multirow{2}{*}{350} & \multirow{2}{*}{3000}\\
\textbf{\racecensus} &  & \\
 \bottomrule
\end{tabular}
\end{center}
\label{tab:efficiency}
\end{table}


==> tables/tab_notations.tex <==
\setlength\tabcolsep{1.5pt}
\begin{table}[!htb]
\footnotesize
\caption{Summary of notations used in this work.}
\footnotesize
\begin{center}
\begin{tabular}{ | c | p{6cm} | }
\hline
\textbf{Notation} & \textbf{Meaning} \\
\hline
 \prover & Prover (e.g., model trainer) \\
 \malprover & Malicious Prover (tries to fool attestation) \\
 \verifier & Verifier (e.g., customer purchasing model, regulator) \\  
 \adv & Adversary (Property Inference Attack) \\
 \hline
 \preq & Required dataset property\\
 \pset & Set of $n$ possible property values \\
$\data$ & Data Distribution \\
$\mathcal{D}_{tr}$ & Training data for model (not specific to our attestation)\\
$\mathcal{G}_0(\data)$, $\mathcal{G}_1(\data)$ & Sub-distributions with specific property (for property inference attacks)\\
\proverdata &  Data split available to prover\\
\verifierdata & Data split available to verifier\\
\verifiertestdata &  Verifier's test dataset \\
\verificationdata &  Dataset for final attestation (taken from prover's data split)\\
\hline
\modelcheck & Model to be attested\\
$\Nmodels$ & Number of shadow models for each values in \pset\\
\modelmpc & Model obtained after secure training with MPC\\
\hline
$\mathcal{N}$ & Total number of provers undergoing attestation\\
$\Naccepts$ & Number of accepted provers\\
\Nspotcheck & Number of spotchecks for fixed FRR in hybrid attestation\\
$\CostInf$ & Cost of inference\\
$\CostCryptComp$ & Cryptographic computation cost (indicated as $\CostCrypt$) \\ 
$\CostCryptComm$ & Cryptographic communication cost (indicated as $\CostCrypt$) \\
$\Pinf$ & Probability of using inference-based attestation\\
$\Pfallback$ & Probability of using cryptographic fallback\\
$\Pspotcheck$ & Probability of conducting a spotcheck\\
\hline
$z$ & Total false accepts from the inference-based attestation\\
% $k$ & Spot-checks from sample of accepted provers\\
$t$ & Number of false accepts from $k$ provers\\
\hline
\end{tabular}
\end{center}
\label{tab:notations}
\end{table}
